Multi-Party Quantum Purity Distillation with Bounded Classical Communication

We consider the task of distilling local purity from a noisy quantum state $\rho^{ABC}$, wherein we provide a protocol for three parties, Alice, Bob and Charlie, to distill local purity (at a rate $P$) from many independent copies of a given quantum state $\rho^{ABC}$. The three parties have access to their respective subsystems of $\rho^{ABC}$, and are provided with pure ancilla catalytically, i.e., with the promise of returning them unaltered after the end of the protocol. In addition, Alice and Bob can communicate with Charlie using a one-way multiple-access dephasing channel of link rates $R_1$ and $R_2$, respectively. The objective of the protocol is to minimize the usage of the dephasing channel (in terms of rates $R_1$ and $R_2$) while maximizing the asymptotic purity that can be jointly distilled from $\rho^{ABC}$. To achieve this, we employ ideas from distributed measurement compression protocols, and in turn, characterize a set of sufficient conditions on $(P,R_1,R_2)$ in terms of quantum information theoretic quantities such that $P$ amount of purity can be distilled using rates $R_1$ and $R_2$. Finally, we also incorporate the technique of asymptotic algebraic structured coding, and provide a unified approach of characterizing the performance limits.

==> Theorem_Distributed_UsingLinearCodes.tex <==
%\section{Simulation of Distributed POVMs with Stochastic Processing}\label{sec:nf_dist_POVM}
%In this section, we dCharlielop a stochastic processing  variant of the distributed POVM simulation problem described in Section \ref{sec:Appx_POVM}. 
% Consider a bipartite composite quantum system $(A,B)$ represented by Hilbert Space $\mathcal{H}_A\tensor \mathcal{H}_B$.
% Let $\rho_{AB}$ be a density operator acting on a composite Hilbert Space  $\mathcal{H}_A\tensor \mathcal{H}_B$.
% Let $\rho_{AB}\in\mathcal{D}(\mathcal{H}_A\tensor\mathcal{H}_B)$. 
Let $\rho_{AB}$ be a density operator acting on  $\mathcal{H}_A\tensor \mathcal{H}_B$.
Consider two measurements $M_A$ and $M_B$ on sub-systems $A$ and $B$, respectively. 
Imagine again that we have three parties, named Alice, Bob and Charlie, trying to collectively simulate a given measurement $M_{AB}$
% = \{\Lambda_z\}_{z\in \mathcal{Z}}$ 
performed on $\rho_{AB}$, as shown in Fig. \ref{fig:NF_Distributed}. Charlie additionally has access to unlimited private randomness.
% The resources available to these parties are: some amount of classical common randomness shared among them, and classical communication links of specified rates between Alice and Charlie, and Bob and Charlie. Further, the operators of the given measurement $M_{AB}$, admit a decomposition of the form $\Lambda_z = \sum_{l_1 \in\mathcal{L}_1}\sum_{l_2\in\mathcal{L}_2}P(z|l_1,l_2)\Lambda_{l_1}\tensor\Lambda_{l_2}; z \in \mathcal{Z}$. The operators $\{\Lambda_{l_1}\}_{l_1 \in\mathcal{L}_1}$ and $\{\Lambda_{l_2}\}_{l_2 \in\mathcal{L}_2}$ correspond to the elements of some POVMs $M_A$ and $M_B$ which Alice and Bob would conventionally perform on the each of the sub-systems of the state $\rho_{AB}$ available to them, and $P(z|l_1,l_2)$ is any stochastic map Charlie is capable of performing. Ideally with no constraints on the rates, Alice and Bob would have sent the outcomes of each of these measurements $M_A$ and $M_B$ to Charlie, who perturbs it using the map $P(z|l_1,l_2)$ which produces an overall effect of $M_{AB}$ acting on $\rho_{AB}$. HowCharlier, with the limited resources available, Alice and Bob instead choose to perform some approximating measurements $\tilde{M}_A$ and $\tilde{M}_B$ on $n$ copies of sub-systems $A$ and $B$, respectively. The measurements are performed in a distributed fashion with no communication taking place between Alice and Bob. Based on their respective measurements and the common randomness, Alice and Bob send some classical bits to Charlie. %In this context, the overall measurement is characterized by the tensor product measurement $M_A \tensor M_B$.  
% 		 Upon receiving these classical bits, Charlie applies a stochastic processing operation on them and, then, wishes to produce an $n$-letter classical sequence. The objective is to construct $n$-letter measurements $\tilde{M}_A$ and $\tilde{M}_B$ that minimize the classical communication and common randomness bits while ensuring that the overall measurement induced by the action of the three parties is close to $M^{\tensor n}_{AB}$.
The problem is formally defined in the following.
		 
% \begin{figure}[hbt]
% 	\begin{center}
% 	  \includegraphics[scale=0.36]{NF_Distributed.png}
%     \caption{The diagram depicting the distributed POVM simulation problem with stochastic processing. In this setting, Charlie additionally has access to unlimited private randomness.}
%     %of a distributed quantum measurement applied to a bipartite quantum system $AB$. A tensor product measurement $M_A\tensor M_B$ is performed on many copies of the observed quantum state. The outcomes of the measurements are given by two classical bits. The receiver functions as a classical-to-quantum channel $\beta$ mapping the classical data to a quantum state.} 
%     \label{fig:NF_Distributed}  
% 	\end{center}
% \end{figure}
\begin{definition}
	For a given finite set $\mathcal{Z}$, and a Hilbert space $\mathcal{H}_{A}\tensor \mathcal{H}_B$, a distributed protocol with stochastic processing with parameters $(n,\Theta_1,\Theta_2,N)$ 
	is characterized by %a collections of POVM-pairs  $\tilde{M}_A^{(\mu)}$ and $\tilde{M}_B^{(\mu)},\mu \in [1, N]$, each 1) acting on $\mathcal{H}_A^{\tensor n}$ and $\mathcal{H}_B^{\tensor n}$, and 2) having at most $\Theta_1$ and $\Theta_2$ outcomes, respectively.
	\\
		\textbf{1)} a collections of Alice's sub-POVMs  $\tilde{M}_A^{(\mu)},\mu \in [1, N]$ each acting on $\mathcal{H}_A^{\tensor n}$ and with outcomes in  $\mathcal{L}_1$ satisfying $|\mathcal{L}_1|\leq \Theta_1$.\\
		\textbf{2)} a collections of Bob's sub-POVMs  $\tilde{M}_B^{(\mu)},\mu \in [1, N]$ each acting on $\mathcal{H}_B^{\tensor n}$ and with outcomes in  $\mathcal{L}_2$, satisfying $|\mathcal{L}_2|\leq \Theta_2$.\\
		\textbf{3)} Charlie's   classical stochastic map $P^{(\mu)}(z^n|l_1, l_2)$ for all $l_1\in \mathcal{L}_1, l_2\in \mathcal{L}_2, z^n\in \mathcal{Z}^n$ and $\mu \in [1,N]$. \\
		The overall  sub-POVM of this distributed protocol, given by $\tilde{M}_{AB}$, is characterized by the following operators:\\ 
		$\tilde{\Lambda}_{z^n}\deq \frac{1}{N}\sum_{\mu, l_1, l_2} P^{(\mu)}(z^n|l_1,l_2)~ \Lambda^{A,(\mu)}_{l_1}\tensor \Lambda^{B,(\mu)}_{l_2}, \quad \forall z^n \in \mathcal{Z}^n,$
% 		\begin{equation}
% 		\tilde{\Lambda}_{z^n}\deq \frac{1}{N}\sum_{\mu, l_1, l_2} P^{(\mu)}(z^n|l_1,l_2)~ \Lambda^{A,(\mu)}_{l_1}\tensor \Lambda^{B,(\mu)}_{l_2}, \quad \forall z^n \in \mathcal{Z}^n, \nonumber
% 		\end{equation}
		where $\Lambda^{A,(\mu)}_{l_1}$ and  $\Lambda^{B,(\mu)}_{l_2}$ are the operators corresponding to the sub-POVMs $\tilde{M}_A^{(\mu)}$ and $\tilde{M}_B^{(\mu)}$, respectively.
	%
	% $M_A^{(n, \mu)}$ and $M_B^{(n, \mu)}),\mu \in [1, 2^{nC}]$ acting on $\mathcal{H}_A^{\tensor n}$ and $\mathcal{H}_B^{\tensor n}$, respectively.
	%
	%
	%1. a collection of POVMs $M_A^{(n, \mu)},\mu \in [1, 2^{nC}]$ acting on $\mathcal{H}_A^{\tensor n}$ with at most $2^{nR_1}$ outcomes. 
	%2. a collection of POVMs $M_B^{(n, \mu)},\mu \in [1, 2^{nC}]$ acting on $\mathcal{H}_B^{\tensor n}$ with at most $2^{nR_2}$ outcomes.
	%3. a collection of mappings  $\beta^{(\mu)}: [1:2^{nR_1}]\times [1:2^{nR_2}] \mapsto \mathcal{X}^n$
	%
	%
	%a collection of $2^{nC}$ POVM-pairs $(M_A^{(n, \mu)}, M_B^{(n, \mu)}),\mu \in [1, 2^{nC}]$ acting on $\mathcal{H}^{\tensor n}_{AB}$ and with at most $2^{nR_1}$ and $2^{nR_2}$ outcomes. mappings $\beta^{(\mu)}: \mathcal{X}^n\mapsto \mathcal{Y}^n$, and 
\end{definition}
% In the above definition,  $(\Theta_1,\Theta_2)$ determines the amount of classical bits communicated from Alice and Bob to Charlie. The amount of common randomness is determined by  $N$. The classical stochastic maps 
% $P^{(\mu)}(z^n|l_1,l_2)$ represents the action of Charlie.
% on the received classical bits.  
\begin{definition}
	Given a POVM $M_{AB}$ acting on  $\mathcal{H}_{A}\tensor \mathcal{H}_B$, and a density operator $\rho_{AB}\in \mathcal{D}(\mathcal{H}_{A}\tensor \mathcal{H}_B)$, a triple $(R_1,R_2,C)$ is said to be achievable, if for all $\epsilon>0$ and for all sufficiently large $n$, there exists a distributed protocol with stochastic processing with parameters  $(n, \Theta_1, \Theta_2, N)$ such that its overall sub-POVM $\tilde{M}_{AB}$  is $\epsilon$-faithful to $M_{AB}^{\tensor n}$ with respect to $\rho_{AB}^{\tensor n}$ (see Definition \ref{def:faith-sim}), and $\frac{1}{n}\log_2 \Theta_i \leq R_i+\epsilon, \quad i=1,2,$ and $	\frac{1}{n}\log_2 N \leq C+\epsilon.$
% 	\begin{align*}
% 	\frac{1}{n}\log_2 \Theta_i \leq R_i+\epsilon, \quad i=1,2, \quad \mbox{and} \quad
% 	\frac{1}{n}\log_2 N \leq C+\epsilon.
% 	\end{align*}
	The set of all achievable triples $(R_1,R_2,C)$ is called the achievable rate region. 
\end{definition}
\begin{definition}[Joint Measurements]\label{def:Joint Measurements}A POVM $M_{AB} = \{\Lambda^{AB}_z\}_{z \in \mathcal{Z}}$, acting on a joint state $\rho_{AB} \in \mathcal{D}(\mathcal{H}_{A}\tensor \mathcal{H}_B)$, is said to have a separable decomposition with stochastic modulo-sum integration  with respect to a prime finite field $\mathbb{F}_p$  if there exist POVMs $\bar{M}_A=\{\bar{\Lambda}^A_{u}\}_{u \in \mathcal{U}}$ and $\bar{M}_B=\{ \bar{\Lambda}^B_{v}\}_{v \in \mathcal{V}}$ and a stochastic mapping $P_{Z|W}: \mathcal{W} \rightarrow\mathcal{Z}$ such that $\Lambda^{AB}_{z}=\sum_{u,v} P_{Z|W}(z|u+ v) \bar{\Lambda}^A_{u}\tensor \bar{\Lambda}^B_{v}, \quad  \forall z \in \mathcal{Z}, \nonumber$
% 	\begin{equation}
% 	\Lambda^{AB}_{z}=\sum_{u,v} P_{Z|W}(z|u+ v) \bar{\Lambda}^A_{u}\tensor \bar{\Lambda}^B_{v}, \quad  \forall z \in \mathcal{Z}, \nonumber
% 	\end{equation}
	where $W = U+ V$, $\mathcal{U}= \mathcal{V}=\mathcal{W}=\FF_p$, with $\FF_p$ being  a prime finite field, and $\mathcal{Z}$ is a finite set.
% 	Further, if the mapping $P_{Z|W}$ is a deterministic function, then the POVM is said to have a separable decomposition with deterministic modulo-sum integration. 
\end{definition}
\vspace{-3pt}
\begin{remark}
% It can be noted that not all joint measurements acting on an entangled state can be simulated faithfully in a distributed fashion. The above measurements are the most general types of joint measurements (acting on an entangled quantum state) that are shown to be simulatable in a distributed setting. 
The measurements considered in \cite{atif2019faithful} had a separable decomposition with stochastic integration. 
% In this work, we have generalized these following the above definition.
% these to joint measurements that have separable decomposition with stochastic modulo-sum integration with respect to a prime finite field. 
% Note that the latter  is a more general definition. This definition, in fact, subsumes the former, as  
% of \cite{atif2019faithful}. This is true because 
Note that the above definition (Def. \ref{def:Joint Measurements}) is more generic and hence subsumes the former, as any non-linear bivariate function can be embedded in a linear function by embedding the input variables into a larger finite field (see \cite[Def. 3.7]{pradhanalgebraic}). 
% For instance, a logical binary OR function (clearly non-linear) over binary inputs can be embedded in the linear function corresponding to the ternary field ().  
\end{remark}
\vspace{-3pt}


The following theorem provides an inner bound to the {achievable} rate region, which is proved in Section \ref{sec:proof of thm dist POVM}.


\begin{theorem}\label{thm:dist POVM appx}
		Given a density operator $\rho_{AB}\in \mathcal{D}(\mathcal{H}_{A}\tensor \mathcal{H}_B)$, and a POVM $M_{AB}=\{\Lambda^{AB}_{z}\}_{z \in \mathcal{Z}}$ acting on  $\mathcal{H}_{A}\tensor \mathcal{H}_B$ having a separable decomposition with stochastic {modulo sum integration with respect to a prime finite field} $\mathbb{F}_p$  (as in Definition \ref{def:Joint Measurements}), yielding POVMs $\bar{M}_A=\{\bar{\Lambda}^A_{u}\}_{u \in \mathcal{U}}$ and $\bar{M}_B=\{ \bar{\Lambda}^B_{v}\}_{v \in \mathcal{V}}$ and a stochastic map $P_{Z|W}:{\FF_p} \rightarrow \mathcal{Z}$ for $\mathcal{U}=\mathcal{V}=\FF_p$ and $W = U+V$, a triple $(R_1,R_2,C)$ is achievable if the following inequalities are satisfied:
			\begin{align}
			R_1 &\geq I(U;R,B)_{\sigma_1}+S(U+ V)_{\sigma_3} - S(U)_{\sigma_3}\nonumber,\\
			R_2 &\geq I(V;R,A)_{\sigma_2}+S(U+ V)_{\sigma_3}-S(V)_{\sigma_3}\nonumber,\\
			R_1 + C &\geq I(U;R,Z,V)_{\sigma_3} +S(U+ V)_{\sigma_3}-S(U)_{\sigma_3}\nonumber ,\\
			R_2 + C &\geq I(V;R,Z)_{\sigma_3} +S(U+ V)_{\sigma_3} -S(V)_{\sigma_3}\nonumber, \\
			R_1+R_2+C &\geq I(U,V;R,Z)_{\sigma_3} \!\!+\! 2S(U+ V )_{\sigma_3} \!\!-\! S(U,V)_{\sigma_3},\nonumber
			\end{align}		
		where $\Psi^{\rho_{AB}}_{R A B}$ is a purification of $\rho_{AB}$, {$ U, V, W$ are defined on $ \mathbb{F}_p$}, and the above information quantities are computed for 
		the auxiliary states
$\sigma_{1}^{RUB} \deq (\emph{id}_R\tensor \bar{M}_{A} \tensor \emph{id}_B) ( \Psi^{\rho_{AB}}_{R A B}), \sigma_{2}^{RAV} \deq (\emph{id}_R\tensor \emph{\id}_A \tensor \bar{M}_{B}) ( \Psi^{\rho_{AB}}_{R A B}),$  
and	$\sigma_3^{RUVZ}   \deq \sum_{u,v,z}\sqrt{\rho_{AB}}\left (\bar{\Lambda}^A_{u}\tensor \bar{\Lambda}^B_{v}\right )\sqrt{\rho_{AB}} \tensor P_{Z|W}(z|u+ v) \ketbra{u}\tensor\ketbra{v}\tensor\ketbra{z},$ for some orthonormal sets $\{\ket{u}\}_{u\in\mathcal{U}}, \{\ket{v}\}_{v\in\mathcal{V}}$, and $\{\ket{z}\}_{z\in\mathcal{Z}}$. 
\end{theorem}
\noindent Note that the rate-region obtained in Theorem 6 of  \cite{atif2019faithful} has the constraint $R_1 + R_2 + C \geq I(U,V;R,Z)_{\sigma_3}$. Hence when $2S(U+V)_{\sigma_3} < S(U,V)_{\sigma_3},$ the above theorem gives a lower sum rate constraint. 
% As a result, the rate-region above contains points that are not contained within the rate-region provided in \cite{atif2019faithful}. 
% An example with detailed illustration is also provided in \cite{atif2021distributed}.
% To illustrate this fact further, consider the following example.
The following example illustrates this fact.

\begin{example}
Suppose the composite state $\rho_{AB} $ is described using one of the Bell states on 
$\mathcal{H}_A\tensor\mathcal{H}_B$ as
% \\$ \rho^{AB} \deq \frac{1}{2}\left(\ket{00}_{AB} + \ket{11}_{AB} \right)\left( \bra{00}_{AB} + \bra{11}_{AB}\right).$
% Let us assume Alice and Bob each receive a quantum particle from an entangled pair of two quantum particles.
% Let the 
% % pair of entangled quantum particles Consider a quantum bipartite particle (say a pair of photons) with its 
% joint state of this entangled pair be described using the Bell state $\Phi^{AB}$ on the Hilbert space $\mathcal{H}_A\tensor\mathcal{H}_B$, where $\Phi^{AB}$ is  given as
\begin{align*}
    \rho^{AB} \deq 1/2\left(\ket{00}_{AB} + \ket{11}_{AB} \right)\left( \bra{00}_{AB} + \bra{11}_{AB}\right).
\end{align*}
% Alice and Bob each have access to the partial sub-systems (A and B, respectively) of the state $\Phi^{AB}$ and hence perceive the 
Since $\pi^A = \Tr_B{\rho^{AB}}$ and $\pi^B = \Tr_A{\rho^{AB}}$, Alice and Bob would perceive each of their particles in maximally mixed states $\pi^A = \frac{I_A}{2}$ and $\pi^B = \frac{I_B}{2}$, respectively. Upon receiving the quantum state, the two parties wish to independently measure their states, using identical POVMs $M_A$ and $M_B$, given by $M_A \deq \left\{ \Lambda_u^A \right\}_{u\in \FF_2}, M_B \deq \left\{\Lambda_v^B\right\}_{v\in\FF_2}$, where $\FF_2$ is a binary field with elements $0$ and $1$, and
\begin{align}
    \Lambda_0^A = \Lambda_0^B = \begin{bmatrix}
                    0.9501 & 0.0826 +i0.1089 \\
                    0.0826 - i0.1089 & 0.0615
                \end{bmatrix}, \quad\nonumber\\
    \Lambda_1^A = \Lambda_1^B = \begin{bmatrix}
                    0.0499 & -0.0826 -i0.1089 \\
                    -0.0826 + i0.1089 & 0.9385
                \end{bmatrix}. \nonumber
\end{align}
Alice and Bob together with Charlie aim to simulate the action of $M_{AB} \deq \left\{\Gamma_z^{AB}\right\}_{z\in\FF_2}$ using the classical communication and common randomness as the resources available to them, where 
\begin{align}
    \Gamma_z^{AB} \deq & \; \lambda_z\left(\Lambda_0^A\tensor\Lambda_0^B + \Lambda_1^A\tensor\Lambda_1^B \right)\nonumber \\ & + (1-\lambda_z)  \left(\Lambda_1^A\tensor\Lambda_0^B + \Lambda_1^A\tensor\Lambda_0^B \right), \text{ for } z \in \FF_2.\nonumber
\end{align} 
Note that $M_{AB}$ admits a separable decomposition  with respect to $\FF_2$ (as per Def. \ref{def:Joint Measurements}), for all $\lambda_z \in (0,1)$, and hence the above theorem gives $    S(U+V)_{\sigma_3} = 0.5155, $ $  S(U)_{\sigma_3} = S(V)_{\sigma_3} = 0.9999,$ $ S(U,V)_{\sigma_3} = 1.5154,$ and $ I(U,V)_{\sigma_3} = 0.4844,$
% \begin{align}
%     S(U+V)_{\sigma_3} = 0.5155, \quad S(U)_{\sigma_3} = S(V)_{\sigma_3} = 0.9999, \quad S(U,V)_{\sigma_3} = 1.5154, \quad I(U,V)_{\sigma_3} = 0.4844,
% \end{align}
where ${\sigma_3}$ is as defined in the statement of Thm. \ref{thm:dist POVM appx}.
Since $S(U)_{\sigma_3}-S(U+V)_{\sigma_3} = S(V)_{\sigma_3}-S(U+V)_{\sigma_3} = I(U,V)_{\sigma_3}, $
 the constraints on $R_1$, $R_2$, $R_1+C$ and $R_2+C$ are the same as obtained in Thm. 6 of \cite{atif2019faithful}. However, with $2S(U+V)_{\sigma_3} - S(U,V)_{\sigma_3} = -0.4844 < 0$, the constraint on $R_1+R_2+C$ in the above theorem  is strictly weaker than the constraint in Thm. 6 of \cite{atif2019faithful}. Therefore, the rate-region obtained above
%  in Theorem \eqref{thm:dist POVM appx} 
is strictly larger than the rate-region in Thm. 6 of \cite{atif2019faithful}. 
%  For further discussion on the comparison of the two rate-regions, see \cite{krithivasan2011distributed}.
% Consider a measurement $M_{AB}$ defined as $M_{AB}\deq M_A\tensor M_B$ which acts on a state $\rho_{AB}\in\mathcal{D}(\mathcal{H}_A\tensor\mathcal{H}_B)$. Let $M_A \deq \{\Lambda_u^A\}_{u\in\FF_2}$ and  $M_B \deq \{\Lambda_v^B\}_{v\in\FF_2}$, where $\FF_2$ denotes a binary field with elements $0$ and $1$. Further, let $M_{AB},$ and $\rho_{AB}$ be such that we obtain the distribution $P_{UV}$ as $P_{UV}(0,0) = 0.003920, P_{UV}(0,1) = 0.976080$ and $P_{UV}(1,0) = 0.019920$. For this, we can compute $S(U+V) = 0.0376223 < \frac{1}{2}S(U,V) = 0.08953145.$

\end{example}
